Co-simulation: State of the art

It is essential to find new ways of enabling experts in different disciplines to collaborate more efficient in the development of ever more complex systems, under increasing market pressures. One possible solution for this challenge is to use a heterogeneous model-based approach where different teams can produce their conventional models and carry out their usual mono-disciplinary analysis, but in addition, the different models can be coupled for simulation (co-simulation), allowing the study of the global behavior of the system. Due to its potential, co-simulation is being studied in many different disciplines but with limited sharing of findings. Our aim with this work is to summarize, bridge, and enhance future research in this multidisciplinary area. We provide an overview of co-simulation approaches, research challenges, and research opportunities, together with a detailed taxonomy with different aspects of the state of the art of co-simulation and classification for the past five years. The main research needs identified are: finding generic approaches for modular, stable and accurate coupling of simulation units; and expressing the adaptations required to ensure that the coupling is correct.

==> extra_deprecated.tex <==
\section{Dynamic Structure A-Causal Co-simulation Scenarios -- Deprecated}

The most general co-simulation scenario we consider is the dynamic structure, a-causal co-simulation scenario, described by:
\begin{equation}\label{eq:cosim_scenario}
\begin{aligned}
& \text{CoSim}=\tuple{T,S,P,\Omega_\text{ext},L} \\
T &  & \text{time base}\\
S=\prod_i S_i &  & \text{simulators}\\
P=P_\text{ext} \times \prod_i P_i   &  & \text{ports}\\
\Omega_\text{ext}=\set{\omega: T \to P_\text{ext}} &  & \text{external input port signal segments}\\
L &  & \text{coupling function}
\end{aligned}
\end{equation}

The time base $T$ is a formalization of the independent variable with a defined ordering relation (partial or total).
We will refer to this variable as the simulated time. 
Notice that the evolution of the simulated time needs not to bear any resemblance to the wall-clock time.
The ports $P$ define the communication mechanism by which the simulation units can communication between each other, and with the environment of the co-simulation scenario.
The set of external ports $P_\text{ext}$ defines the possible inputs or outputs of the co-simulation scenario that connect it to the environment.
The values $\Omega_\text{ext}$ communicated by the environment over the simulated time are known.

Each simulation unit $S_i$ has ports, state and a state transition function:
\begin{equation}
\begin{aligned}
& S_i=\tuple{T,P_i,\Omega_i, Q_i, \delta_i, \lambda_i} \\
P_i &  & \text{port tuple set}\\
\Omega_i=\set{\omega: T \to P_i} &  & \text{input port signal segments}\\
Q_i &  & \text{state set}\\
\delta_i: \Omega_i \times Q_i \to Q_i &  & \text{state transition function}\\
\lambda_i: P_i \times Q_i \to P_i &  & \text{output function}
\end{aligned}
\end{equation}

The port tuple set defines the inputs/outputs that connect the simulation unit to its environment.
In the most general setting, inputs are not distinguished from outputs and, throughout the co-simulation, these may be rearranged.
The $\Omega_i$ set comprises the possible port signals to be used as inputs over time and the $\lambda_i$ function defines how the output signals can be obtained from the state of the simulation unit and its inputs.
The behavior trace of a simulation unit can then be defined as the evolution of the state set $\Omega_i$ together with the evolution of the port set $P_i$ over time.

The coupling function $L$ induces the equation
$$
L(t, P_\text{ext}, P_1, \ldots, P_n) = 0
$$
which couples the external ports and the ports of the simulation units.

In the most general sense, $L$ is time variant, which means that inputs and outputs of the simulation units (and of the co-simulation scenario) may change over time.
This captures two dimensions in a co-simulation scenario classification: \textbf{dynamic/static structure} and \textbf{(a-)causal}.

A co-simulation trace is the Cartesian product of the behavior traces of each simulation unit, together with the evolution of the values of $P_\text{ext}$.

The task of an orchestrator is to compute a co-simulation trace for the co-simulation scenario of Equation \ref{eq:cosim_scenario}. Hence, the orchestrator is nothing but the solver of a simulation scenario. A co-simulation unit is then the composition of a co-simulation scenario with a specific orchestrator.
The following generic method is a possible mechanism for a dynamic structure a-causal co-simulation:

\begin{algorithm}[H]
 \KwData{Stop time $T_f$, a co-simulation scenario \tuple{T,S,P,\Omega_\text{ext},L} and a time increment $H$.}
 \KwResult{A co-simulation.}
 $t := 0$\;
 \While{$t < t_f$}{
	 Solve the following system of equations for the unknowns $\tilde{p}_i$ and $\tilde{p}_\text{ext}$ at time $t$:\\
	 $
	 \system{
		 \begin{matrix}
			 \bar{p}_i &= \lambda_i(\tilde{p}_i, q_i), \text{ for } i=1,\ldots,n \\
			 0 &= L(t, \bar{p}_\text{ext},\tilde{p}_\text{ext}, \bar{p}_1, \tilde{p}_1 , \ldots, \bar{p}_n, \tilde{p}_n)
		 \end{matrix}
	 }
	 $\;
	 The values $\bar{p}_\text{ext},\tilde{p}_\text{ext}, \bar{p}_1, \tilde{p}_1 , \ldots, \bar{p}_n, \tilde{p}_n$ denote a point at time $t$ of the co-simulation trace\;
	 Compute the next state of each simulation unit based on the signal $\omega_i$, extrapolated in the vicinity of $\tilde{p}_i$:\\
	 $\bar{q}_i := \delta_i(\omega_i, q_i), \text{ for } i=1,\ldots,n$\;
	 Advance time:\\
	 $t := t + H$
 }
 \caption{Generic orchestrator.}
\end{algorithm}

Variable $t$ denotes the simulation time and $H>0$ denotes the communication step size.
At each time point, the port tuple of each simulation unit is split into two tuples: $\tilde{p}_i$ and $\bar{p}_i$. 
Whether $\tilde{p}_i$ are inputs and $\bar{p}_i$ outputs (and vice versa) depends on the function $\lambda_i$ and on the coupling function.

The above method is by no means the only orchestrator possible. It represents a basic example to give the reader an intuitive notion of the main tasks of an orchestrator: move and approximate data between ports according to the coupling function, advance the state of each simulation unit and the simulation time.

For industrial applications, the \textbf{run-time performance} of the co-simulation unit is important. It is measured by the amount of wall-clock time spent $\Delta W$ computing the co-simulation trace over a predefined interval of simulation time $\Delta T$.
In as-fast-as-possible co-simulations, there is no relation between $\Delta W$ and $\Delta T$: the co-simulation unit advances through $T$ as fast as the executing platform permits. In real-time co-simulations, the ratio $\frac{\Delta W}{\Delta T}=1$. In scaled real-time co-simulation, the ratio $\frac{\Delta W}{\Delta T}=f(t)$ where $f(t)$ can either be a constant (fixed scale) or a continuous function of the simulation time $t \in T$.

It is not hard to see that, with the definition of co-simulation scenario and simulation unit, a co-simulation scenario, together with a solver, can be written as a simulation unit with the output function being the Cartesian product of the values of all ports.
Should we do that? Or is it obvious?
This captures a dimension in co-simulation classification: \textbf{hierarchy}.

Furthermore, it begs the question: What is a correct co-simulation scenario?
Since a co-simulation scenario is a simulation unit, it must be accurate and the model it is simulating must be valid.

The model being simulated by a co-simulator is the coupling of the models being solved by each simulation unit in the scenario, defined by the coupling function $L$.
Assuming that the sub-models are valid, then the coupled model is valid if and only if the coupling function is valid.
Judging the validity of the coupling function is an open challenge in the field of modeling.

By similar reasoning, assuming the simulation units are accurate, then the co-simulation unit is accurate if and only if it can accurately solve the coupling equation over time.
For the above example method, the accuracy depends on the accuracy of the solution to $L$ and on the extrapolation method used to get $\omega_i$, which in turn depends on the communication step size $H$.
This is generally the case for any method.

These matters of validity and accuracy highlight another dimension in co-simulation: \textbf{compositionality}. How can properties (validity, accuracy, etc\ldots) satisfied by every simulation units in a co-simulation scenario, also be satisfied by the scenario itself?






==> nfr.tex <==
%%>>>> Begin Generated Code: cat=nfr:accuracy
%%<<<< End Generated Code



==> simulator_capabilities.tex <==
\section{Simulation Unit Capabilities}

This chapter is concerned with organizing the capabilities of each simulation unit.

\subsection{Availability}

\subsubsection{Remote}

Available as a web service.

\subsubsection{Local}

Available in binary or source code form to be executed locally.

\paragraph{Binary}
\label{capabilities:sr:info:availability:local:binary}

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\paragraph{Source}
\label{capabilities:sr:info:availability:local:source}

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\subsection{Causality}

\subsubsection{Causal}
\label{capabilities:sr:info:causality:causal}

	Input/Output directionality is predefined.

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\subsubsection{A-Causal}

	I/O directionality is not predefined.

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code



\subsection{Simulation Parameters}

\subsubsection{Fixed}
\label{capabilities:sr:info:parameters:fixed}

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\subsubsection{Tunable}

\subsection{Rollback Support}

\subsubsection{None}
\label{capabilities:info:rollback:none}

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code


\subsubsection{Single}
\label{capabilities:info:rollback:single}

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\subsubsection{Multiple}
\label{capabilities:sr:info:rollback:multiple}

\subsection{Time Model}

The contents of this section can be expanded by reading \cite{Furia2008}.

\subsubsection{Linear Time}
\label{capabilities:sr:info:time:linear}

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\subsubsection{Branching Time}

\paragraph{Non-Deterministic}

\paragraph{Stochastic}

\subsection{Time Constraints}

\subsubsection{Unconstrained}
\label{capabilities:sr:info:time_constraints:none}

Allows for analytic simulation.

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\subsubsection{Scaled Real Time}

\paragraph{Static}

This is constrained to have a fixed relation with respected to the real-time.

\paragraph{Dynamic}

A variable relation is kept with respect to real time.
This allows the simulation to slow down and go faster depending on the signals (e.g., for debugging purposes).

\subsection{Step Size}

\subsubsection{Fixed Step Size}
\label{capabilities:sr:info:step_size:fixed}

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\subsubsection{Dynamic Step Size}
\label{capabilities:sr:info:step_size:adaptive}


\paragraph{Changeable}
\label{capabilities:sr:info:step_size:adaptive:changeable}

The ability to set the simulator's next step size. He might reject that but this is still an important capability to enable state event detection.

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code

\paragraph{Unchangeable}


\subsubsection{Straggler Event Detection Support}
\label{capabilities:sr:info:error_detect:straggler}

This represents the ability to signal an error when an event is processed with a time stamp inferior to the current time of the simulation unit.

%%>>>> Begin Generated Code
References in this category:

Tools in this category:

%%<<<< End Generated Code











==> state_of_art_tocover.tex <==
\section{State of the Art in Co-simulation Not Classified}

This section includes all references that we still need to cover.

\subsection{Papers}

\begin{Reference}{A Gluing Algorithm for Distributed Simulation of Multibody Systems}{Wang2003}
TODO.

From other reads:
They introduce a gluing algorithm that couples ‘‘in a plug-and-play manner’’ different component models in
the simulation of multibody systems. Their algorithm assumes that partitioning is not controlled by the user and focuses
exclusively on how to make the partitions communicate (i.e., exchange interface information) during simulations.
\end{Reference}

\begin{Reference}{Virtual integration of Automotive Hard-and Software with Silver}{Junghanns2010}
TODO.
\end{Reference}


\begin{Reference}{A multilevel Newton algorithm with macromodeling and latency for the analysis of large-scale nonlinear circuits in the time domain}{Rabbat1979}
TODO.
Might give us ideas about analysis support categories.
\end{Reference}

\begin{Reference}{Co-Simulation of Hybrid Systems: Signal-Simulink}{Tudoret2000}
TODO.
\end{Reference}

\begin{Reference}{"Leapfrog" methods for numerical solution of differential equations, sinewave generation, and magnitude approximation}{Nelson1995}
TODO.
\end{Reference}




\begin{Reference}{A SystemC/Simulink Co-Simulation Framework for Continuous/Discrete-Events Simulation}{Bouchhima2006}
TODO.
\end{Reference}




\begin{Reference}{Efficient Multirate Simulation of Complex Multibody Systems Based on Free Software}{Solcia2011}

\end{Reference}






\begin{Reference}{Automatic Generation of a Coverification Platform}{Kajtazovic2006}
They present a coupling of several simulators from both discrete-event and continuous time simulation with the purpose of co-simulating microelectronic embedded systems.
The orchestration method they use is a well known conservative discrete event simulators and their contribution is in the automatic generation of the interfaces that wrap a continuous time simulator as a DE system.
This means they get distribution and parallelism for free.
Also, the wrapped simulator do not need to support rollback.
There is organization of simulators into cluster, but this is dependent on their type, and little though is given into optimizing for performance or accuracy.
They used a car power management system as a case study.
The correct behavior trace that they used to measure the error in the co-simulation is computed from the coupled model, solved by a single tool.

\catref{nfr:ip_protection}
\catref{nfr:parallelism}
\catref{nfr:distribution}
\catref{nfr:extensibility} % They explicitly mention this and present it in the paper.
\catref{sr:causality:causal}
\catref{fr:num_sim:three_more}
\catref{fr:domain:de}
\catref{sr:availability:remote}
\catref{fr:coupling_model:io_assignments}
\catref{sr:rollback:none}
\catref{sr:rel_time:analytic}
\catref{fr:sim_rate:multi}
\catref{fr:sim_step_size:variable}
\catref{fr:alg_loop:explicit}
\catref{fr:results_visualization:post_mortem}
\catref{fr:communication_model:gauss_seidel}
\end{Reference}

\begin{Reference}{Accuracy-adaptive Simulation of Transaction Level Models}{Radetzki2008}
TODO.
\end{Reference}

\begin{Reference}{Multi-Accuracy Power and Performance Transaction-Level Modeling}{Beltrame2007}
This is about multi-level simulation.
It gives us ideas to be applied in co-simulation.
TODO.
\end{Reference}

\begin{Reference}{Optimizing communication in embedded system co-simulation}{Hines1997b}
TODO.
\end{Reference}

\begin{Reference}{Selective focus as a means of improving geographically distributed embedded system co-simulation}{Hines1997}
TODO.
\end{Reference}

\begin{Reference}{Dynamic Communication Models in Embedded System Co-simulation}{Hines1997a}
TODO.
\end{Reference}

\begin{Reference}{Physically oriented modeling of heterogeneous systems}{Schwarz2000}
TODO.
Might give us ideas about hierarchical co-simulation.
\end{Reference}



\begin{Reference}{Process Save Reduction by Macro Joint Approach: The Key to Real Time and Efficient Vehicle Simulation}{Eichberger2004}
TODO.
They apply a non-linear model reduction method to the tire suspension system and show the benefits of it.
This might give us ideas about information exposed by the simulation units.
\end{Reference}

\begin{Reference}{Verification of Analog and Mixed-Signal Circuits Using Hybrid System Techniques}{Dang2004}
TODO.
Will give us ideas for the analysis support category.
\end{Reference}

\begin{Reference}{Towards Formal Verification of Analog Designs}{Gupta2004}
TODO.
They apply model checking techniques to continuous models.
This might give us ideas for analysis support categories.
\end{Reference}


\begin{Reference}{Modeling of combined discrete/continuous processes}{Barton1994}
A mathematical description of the combined discrete/continuous simulation problem is introduced to enhance the understanding of the fundamental discrete changes required to model processing systems.
TODO.
\end{Reference}

\begin{Reference}{Modeling, simulation, sensitivity analysis, and optimization of hybrid systems}{Barton2002}
TODO.
\end{Reference}

\begin{Reference}{Dynamic optimization of hybrib systems}{Galan1998}
TODO.
This paper presents a problem formulation and a preliminary classification, some mathematical results on hybrid dynamic optimization.
It might give us ideas for analysis techniques and information exposed about the simulation units.
\end{Reference}

\begin{Reference}{A companion model approach to modelling and simulation of industrial processes}{Juslin2005}
This is a book.
TODO.
\end{Reference}

\begin{Reference}{Interval and point-based approaches to hybrid system verification}{Kapur1997}
TODO.
\end{Reference}

\begin{Reference}{Heterogeneous Simulation — Mixing Discrete-Event Models with Dataflow}{Lee1997}
TODO.
\end{Reference}


\begin{Reference}{Hidden discontinuities and parametric sensitivity calculations}{Tolsma2002}
TODO.
Might give us some ideas for the analysis and simulation unit categories.
\end{Reference}

\begin{Reference}{Bridging the Semantic Gap Between Heterogeneous Modeling Formalisms and FMI}{Tripakis2014}
\cite{Tripakis2014} discuss how to create different FMUs
from heterogeneous modeling formalisms. They formally define how to encode an
FMU and which adaptations are required for certain classes of formalisms, for
example timed and un-timed formalisms.
This will give us ideas about the simulation units capabilities.
\end{Reference}

\begin{Reference}{Operational semantics of hybrid systems}{Zheng2007}
They present interesting test cases for co-simulation.
TODO.
\end{Reference}

\begin{Reference}{Closing the gap between UML-based modeling, simulation and synthesis of combined HW/SW systems}{Mischkalla2010}
TODO.
\end{Reference}

\begin{Reference}{Co-simulation Tools for Networked Control Systems}{Al-Hammouri2008}
TODO.
\end{Reference}

\begin{Reference}{Co-synthesis and co-simulation of control-dominated embedded systems}{Balboni1996}
TODO.
\end{Reference}




\begin{Reference}{Discrete-continuous simulation model for accurate validation in component-based heterogeneous SoC design}{Bouchhima2005}
TODO.
\end{Reference}






\begin{Reference}{On model-driven design of robot software using co-simulation}{Broenink2010} 
TODO.
\end{Reference}



\begin{Reference}{Efficient Optimistic Parallel Simulations Using Reverse Computation}{Carothers1999a}
TODO.
Might give us ideas on synchronization methods.
\end{Reference}


\begin{Reference}{Component-Based Hardware/Software Co-Simulation}{Cheung2007}
TODO.
\end{Reference}

\begin{Reference}{Multilanguage design of heterogeneous systems}{Coste1999}
TODO.
\end{Reference}

\begin{Reference}{Improving the Composability of DoD Models and Simulations}{Davis2004}
TODO.
Discusses ideas for improving the composability of future models and simulations developed or used by the U.S. Department of Defense.
Might give us ideas about information for simulation units.
\end{Reference}


\begin{Reference}{Verilog-AMS: Mixed-signal simulation and cross domain connect modules}{Frey2000c}
TODO.
\end{Reference}

\begin{Reference}{Scalable and flexible cosimulation of SoC designs with heterogeneous multi-processor target architectures}{Gerin2001}
TODO.
\end{Reference}

\begin{Reference}{An Effective VHDL-AMS Simulation Algorithm with Event Partitioning}{Ghasemi2005a}
TODO.
\end{Reference}

\begin{Reference}{Formal Definitions of Simulation Interfaces in a Continuous/Discrete Co-Simulation Tool}{Gheorghe2006}
TODO.
\end{Reference}

\begin{Reference}{A Formalization of Global Simulation Models for Continuous/Discrete Systems}{Gheorghe2007}
TODO.
\end{Reference}

\begin{Reference}{Semantics for Model-based Validation of Continuous/Discrete Systems}{Gheorghe2008a}
TODO.
\end{Reference}

\begin{Reference}{Semantics for Rollback-Based Continuous/Discrete Simulation}{Gheorghe2008}
TODO.
\end{Reference}

\begin{Reference}{Modeling Smart Grid Applications with Co-Simulation}{Godfrey2010}
TODO.
\end{Reference}





\begin{Reference}{Co-simulation framework for Networked Control Systems over multi-hop mobile ad-hoc networks}{HASAN2008}
TODO.
\end{Reference}

\begin{Reference}{Using ModelSim, Matlab/Simulink and NS for Simulation of Distributed Systems}{Hatnik2004}
TODO.
\end{Reference}

\begin{Reference}{Mixed-signal simulation with the Simbus backplane}{Hickey2006}
TODO.
\end{Reference}

\begin{Reference}{EPOCHS: a platform for agent-based electric power and communication simulation built from commercial off-the-shelf components}{Hopkinson2006}
TODO.
\end{Reference}

\begin{Reference}{Real-time multirate synchronous simulation with single and multiple processors}{Howe1998}
TODO.
\end{Reference}

\begin{Reference}{EM/Circuit Co-Simulation: A Highly Accurate Method for Microwave Amplifier Design}{Kassim2010}
TODO.
\end{Reference}

\begin{Reference}{Simulation of complex systems using Modelica and tool coupling}{Kossel2006}
TODO.
\end{Reference}

\begin{Reference}{Modular Simulation in Multibody System Dynamics}{Kubler2000a}
TODO.
The modular simulation of the global system by coupling of simulators may result in an unstable integration if an algebraic loop exists between the subsystems. 
This numerical phenomenon is analyzed and a method of simulator coupling which guarantees stability for general systems including algebraic loops is introduced.
\end{Reference}

\begin{Reference}{Two Methods of Simulator Coupling}{Kubler2000}
They present a semi-informal representation of co-simulation for continuous time systems.
They define and study the zero-stability of two possible couplings for co-simulation and they exemplify the application of these methods with a double pendulum.
They also show the application of filters to get rid of algebraic loops.
They conclude by arguing that, for stability reasons, iterative techniques are preferred when dealing with black box tools.
\end{Reference}

\begin{Reference}{Hardware, software and mechanical cosimulation for automotive applications}{LeMarrec1998}
TODO.
\end{Reference}


\begin{Reference}{Integrating multiple parallel simulation engines for mixed-technology parallel simulation}{Martin2002}
TODO.
\end{Reference}

\begin{Reference}{Analysis of the intervertebral discs adjacent to interbody fusion using a multibody and finite element co-simulation}{Monteiro2009}
TODO.
\end{Reference}

\begin{Reference}{Agents and Artefacts for Multiple Models Co-evolution: Building Complex System Simulation As a Set of Interacting Models}{Siebert2010}
TODO.
\end{Reference}

\begin{Reference}{Validation in a Component-based Design Flow for Multicore SoCs}{Nicolescu2002}
TODO.
\end{Reference}

\begin{Reference}{CODIS A framework for continuous/discrete systems co-simulation}{Nicolescu2006}
TODO.
\end{Reference}

\begin{Reference}{Methodology for efficient design of continuous/discrete-events co-simulation tools}{Nicolescu2007}
TODO.
\end{Reference}

\begin{Reference}{Mixed-level Cosimulation for Fine Gradual Refinement of Communication in SoC Design}{Nicolescu2001}
TODO.
\end{Reference}

\begin{Reference}{Application of Multi-domain and Multi-language Cosimulation To an Optical MEM Switch Design}{Nicolescu2002a}
TODO.
\end{Reference}


\begin{Reference}{Towards a heterogeneous simulation kernel for system-level models: a SystemC kernel for synchronous data flow models}{Patel2005}
TODO.
\end{Reference}

\begin{Reference}{Asynchronous method for the coupled simulation of mechatronic systems}{Petridis2008}
TODO.
\end{Reference}




\begin{Reference}{Methodology for hardware/software co-verification in C/C++ }{Semeria2000}
TODO.
\end{Reference}


\begin{Reference}{SystemCSV - an extension of SystemC for mixed multi-level communication modeling and interface-based system design}{Siegmund2001}
TODO.
\end{Reference}


\begin{Reference}{Co-simulation of networked embedded control systems, a CSP-like process-oriented approach}{TenBerge2006}
TODO.
\end{Reference}

\begin{Reference}{Co-simulation for performance prediction of integrated building and HVAC systems – An analysis of solution characteristics using a two-body system}{Trcka2010}
TODO.
\end{Reference}

\begin{Reference}{Automatic VHDL-C Interface Generation for Distributed Cosimulation: Application to Large Design Examples}{Valderrama1998}
TODO.
\end{Reference}

\begin{Reference}{A new synchronization algorithm for VHDL-AMS simulation}{Xiao2002}
TODO.
\end{Reference}

\begin{Reference}{A structuring mechanism for embedded control systems using co-modelling and co-simulation}{Zhang2012}

\end{Reference}

\begin{Reference}{Virtual prototyping through co-simulation of a Cartesian plotter}{Groothuis2008}
They motivate well the need for generative approaches for co-simulation and the difficulty in supporting different formalisms if the co-simulation framework is ad-hoc. CoSiMate supports a wide range of formalisms: ModelSim (VHDL), C, SystemC, Simulink, StateMate and Saber.
TODO.
\end{Reference}

\begin{Reference}{A hardware-software co-simulator for embedded system design and debugging}{Ghosh1995}
They provide a flexible and simulator independent backplane where new simulators can be easily integrated.
	The synchronization mechanism is based in the lock step approach but it is unclear how certain challenges such as struggler events are handled. It seems that it is a sequential approach.
TODO.
\end{Reference}

\begin{Reference}{Generic discrete–continuous simulation model for accurate validation in heterogeneous systems design}{Bouchhima2007}
	They present a continuous/discrete co-simulation model between SystemC and Simulink. The CODIS tool.
	The co-simulation architecture is generic but they only implement between SystemC and Simulink.
	The co-simulation interfaces are generated and they provide for accurate state event detection.
	The case study they use is a arm controlled by a discrete controller and the continuous component representing the arm.
\end{Reference}

\begin{Reference}{VHDeLDO: A new mixed mode simulation}{ElTahawy1993}
Their model is at the physical level and is based on the lock-step approach.
The execution is sequential.
TODO.
\end{Reference}

\begin{Reference}{Anatomy of a simulation back-plane}{Zwolinski1995}
Develop a collection of functions that allow simulators to exchange data.
	They also present a synchronization algorithm between any number of simulators but that runs sequentially.
TODO.
\end{Reference}

\begin{Reference}{A mixed-signal, functional level simulation framework based on SystemC for system-on-a-chip applications}{Bonnerud2001}
They give a deeper understanding of the problems involved in co-simulation.
TODO.
\end{Reference}

\begin{Reference}{Mixed-signal Modelling in VHDL for System-on-chip}{Pichon1995}
TODO.
\end{Reference}

\begin{Reference}{SystemC extensions for mixed-signal system design}{Einwich2001}
TODO.
They talk about a synchronization scheme
\end{Reference}

\begin{Reference}{Optimistic synchronization of mixed-mode simulators}{Frey1998}
TODO.
\end{Reference}

\begin{Reference}{Parallel Mixed-technology Simulation}{Frey2000b}
TODO.
\end{Reference}


\begin{Reference}{Behavioral simulation for analog system design verification}{Antao1995}
I think they present a continuous simulation tool called ARCHSIM.
It is not a co-simulation tool but they seem to have a range of useful analysis that we can use to enrich our categorization.
TODO.
\end{Reference}


\begin{Reference}{Performance improvement of geographically distributed co-simulation by hierarchically grouped messages}{Yoo2000}
TODO.
\end{Reference}

\begin{Reference}{Optimistic distributed timed co-simulation based on thread simulation model}{Yoo1998}
TODO.
\end{Reference}



\begin{Reference}{A Framework for Performance Analysis of Parallel Discrete Event Simulators}{Balakrishnan1997}
This seems to be useful for our performance information category.
TODO.
\end{Reference}

\begin{Reference}{Waveform Relaxation Techniques for Simulation of Coupled Interconnects With Frequency-Dependent Parameters Hybrid Systems}{Nakhla2007}
TODO.
\end{Reference}

\begin{Reference}{A Cross Domain Co-Simulation Platform for the Efficient Analysis of Mechatronic Systems}{Karner2010}
The paper introduces the project TEODACS, which contains a framework for co-simulation of mechatronics systems called FlexRayXpert.Sim. This is followed by an introduction of mechatronics systems including descriptions of both the microelectronics domain and the mechanics domain, where the important concepts are presented. Furthermore, the article also describes the tools used for simulating microelectronics and tools used for simulating mechanics. 
One of the biggest issues in this coupling these domains in a co-simulation is the different time bases. A typical microelectronics simulation uses time steps down to picoseconds and an observation range of milliseconds, whereas the mechanics domain has time steps of typically one millisecond and an observation range of seconds or minutes. To address this issue TEODACS makes use of run-time switched co-simulation. Run-time switched co-simulation switches models during the co-simulation to use more complex models and lower speed when relevant effects for microelectronics happens, otherwise a faster simulation speed can be used.
The paper also describes how the data exchange is performed between CarMaker/AVL InMotion and SyAD. A use case based on a Drive-by-Wire application based on FlexRay is presented, that also makes use of FlexRay.Lab, which is a hardware prototype platform.

As this tool is already presented and described in the reference for Heterogeneous co-simulation platform for the efficient analysis of FlexRay-based automotive distributed embedded systems it will not be described further here.
\end{Reference}
\subsection{Tools}

\begin{Tool}{ModelCenter}{modelcenter}
\url{http://www.phoenix-int.com/modelcenter/integrate.php}
\end{Tool}

\begin{Tool}{ISIGHT}{isight}
\url{http://www.3ds.com/products-services/simulia/products/isight-simulia-execution-engine/latest-release/}
\end{Tool}

\begin{Tool}{Adams co-simulation interface}{adamscosiminterface}
TODO.
\end{Tool}

\begin{Tool}{Fraunhofer Co-Simulation Master}{fraunhofer}
TODO.
\end{Tool}

\begin{Tool}{EXITE, EXITE ACE}{exite}
TODO.
\end{Tool}


\begin{Tool}{Advanced Design System}{advancedsystemdesign}
TODO.
\end{Tool}

\begin{Tool}{Command and Control Wind Tunnel (C2WT)}{c2wt}

\catref{nfr:platform_independence}
\catref{nfr:distribution}
\catref{fr:domain:ct}
\catref{fr:num_sim:three_more}
\catref{fr:sim_rate:multi}
\catref{fr:sim_step_size:fixed}
\catref{sr:rel_time:dy_real_scaled_time_simulation}

\end{Tool}

\begin{Tool}{Advanced Process Engineering Co-Simulator (APECS).}{apecs}
TODO.
\end{Tool}

\begin{Tool}{Amesim (from Siemens PLM Software).}{amesim}
TODO.
\end{Tool}

\begin{Tool}{AVL Cruise.}{avlcruise}
TODO.
\end{Tool}

\begin{Tool}{BCVTB}{bcvtb}
TODO.
\end{Tool}

\begin{Tool}{CarMaker}{carmaker}
TODO.
\end{Tool}

\begin{Tool}{Autofocus 3.}{autofocus3}
TODO.
\end{Tool}

\begin{Tool}{CATIA}{catia}
TODO.
This tool uses FMI, according to \refref{Blochwitz2012}.
\end{Tool}

\begin{Tool}{CCSS Co-simulation platform (IBM).}{ccssibm}
TODO.
\end{Tool}

\begin{Tool}{ICOS (Virtual Vehicle)}{icos}
TODO.
Virtual Vehicle Research and Test Center
Papers:
\refref{Krammer2014}
\refref{Krammer2015}
\refref{Krammer2015a}

According to \refref{Krammer2015}, the independent co-simulation framework uses software components called wrappers to establish connections to its supported simulation tools and underlying models.
According to \refref{Krammer2015a}, the co-simulation framework implements the FMI standard.

Categories:
\catref{nfr:config_reusability}
\catref{nfr:parallelism}
\catref{nfr:hierarchy}
\catref{nfr:ip_protection}
\catref{nfr:extensibility}
\catref{fr:domain:ct}
\catref{fr:num_sim:three_more}
\catref{sr:rel_time:analytic}
\catref{sr:availability:local}
\catref{fr:results_visualization:post_mortem}
\catref{sr:info:full_model}
\catref{sr:info:causality:feedthrough}
\end{Tool}

\begin{Tool}{CoCentric.}{cocentric}
TODO.
\end{Tool}

\begin{Tool}{Cocotb.}{cocotb}
TODO.
\end{Tool}

\begin{Tool}{Controluild.}{controluild}
TODO.
\end{Tool}

\begin{Tool}{COSIMATE.}{cosimate}
TODO.
\end{Tool}

\begin{Tool}{CoSimLab.}{cosimlab}
TODO.
\end{Tool}

\begin{Tool}{CoSim (from ICSA).}{cosim}
TODO.
\end{Tool}

\begin{Tool}{CST EM STUDIO.}{cststudio}
TODO.
\end{Tool}

\begin{Tool}{CustomSim (from synopsys).}{customsim}
TODO.
\end{Tool}

\begin{Tool}{Cybernetica ModelFit.}{modelfit}
TODO.
\end{Tool}

\begin{Tool}{DACCOSIM.}{daccosim}
TODO.
\end{Tool}

\begin{Tool}{DevEM (from Magwell).}{devem}
TODO.
\end{Tool}

\begin{Tool}{dSPACE SCALEXIO.}{scalexio}
TODO.
\end{Tool}

\begin{Tool}{dSPACE SYNECT.}{synect}
TODO.
\end{Tool}

\begin{Tool}{dSPACE VEOS.}{veos}
TODO.
\end{Tool}

\begin{Tool}{Dymola.}{dymola}
TODO.
\end{Tool}

\begin{Tool}{EnergyPlus.}{energyplus}
TODO.
According to \refref{Blochwitz2012}, this is a building simulation tool.
\end{Tool}

\begin{Tool}{Enhanced Multiphysics Interface Research Engine (EMPIRE).}{empire}
TODO.
\end{Tool}

\begin{Tool}{ETAS -- INCA-FLOW.}{icaflow}
TODO.
\end{Tool}

\begin{Tool}{ETAS -- LABCAR-OPERATOR}{labcar}
TODO.
\end{Tool}

\begin{Tool}{FLEXICON.}{flexicon}
TODO.
\end{Tool}

\begin{Tool}{Flux (from CEDRAT).}{flux}
TODO.
\end{Tool}

\begin{Tool}{FMI Add-in for EXCEL.}{fmiexcel}
TODO.
\end{Tool}

\begin{Tool}{FMI Add-on fo NI VeriStand.}{addonveristand}
TODO.
\end{Tool}

\begin{Tool}{FMI Blockset for Simulink.}{fmisimulink}
TODO.
\end{Tool}

\begin{Tool}{FMI Library.}{fmilib}
TODO.
\end{Tool}

\begin{Tool}{FMI Toolbox for CarMaker.}{tollboxcarmaker}
TODO.
\end{Tool}

\begin{Tool}{FMI Toolbox for MATLAB/Simulink.}{matlabsimlink}
TODO.
\end{Tool}

\begin{Tool}{FMUSDK.}{fmusdk}
TODO.
\end{Tool}

\begin{Tool}{FNCS.}{fncs}
TODO.
\end{Tool}

\begin{Tool}{ForSyDe.}{forsyde}
TODO.
\end{Tool}

\begin{Tool}{GT-SUITE}{gtsuite}
TODO.
\end{Tool}

\begin{Tool}{HSIMplus HDL Co-simulation.}{hsimplus}
TODO.
\end{Tool}

\begin{Tool}{IGNITE}{ignite}
TODO.
\end{Tool}

\begin{Tool}{JavaFMI}{javafmi}
TODO.
\end{Tool}

\begin{Tool}{JFMI}{jfmi}
TODO.
According to \refref{Blochwitz2012}, this tool is a java Wrapper for FMI, created by the Lawrence Berkeley National Laboratory (LBNL) and UC Berkeley.
\end{Tool}

\begin{Tool}{JModelica}{jmodelica}
TODO.
\end{Tool}


\begin{Tool}{LearnGreenBuildings}{learngreenbuildings}
TODO.
\end{Tool}


\begin{Tool}{LabVIEW}{labview}
TODO.
\end{Tool}

\begin{Tool}{LMS Virtual.Lab Motion}{virtuallabmotion}
TODO.
\end{Tool}

\begin{Tool}{MATLAB}{matlab}
TODO.
\end{Tool}

\begin{Tool}{Modelithics}{modelithics}
TODO.
\end{Tool}

\begin{Tool}{Mosaik}{mosaik}
TODO.
\end{Tool}

\begin{Tool}{MpCCI}{mpcci}
TODO.
\end{Tool}

\begin{Tool}{MyHDL}{myhdl}
TODO.
\end{Tool}

\begin{Tool}{MOKA}{MOKA}
TODO.
\end{Tool}

\begin{Tool}{ns-3}{ns3}
TODO.
\end{Tool}

\begin{Tool}{NX CAE (from Siemens)}{nxcae}
TODO.
\end{Tool}

\begin{Tool}{OpenModelica}{openmodelica}
TODO.
\end{Tool}

\begin{Tool}{PyFMI}{pyfmi}
TODO.
\end{Tool}

\begin{Tool}{RecurDyn}{recurdyn}
TODO.
\end{Tool}

\begin{Tool}{RT-LAB Orchestra}{orchestra}
TODO.
\end{Tool}

\begin{Tool}{Saber}{saber}
TODO.
\end{Tool}

\begin{Tool}{Silver}{silver}
TODO.
\end{Tool}

\begin{Tool}{SimCoupler}{coupler}
TODO.
\end{Tool}

\begin{Tool}{SIMPACK}{pack}
TODO.
\end{Tool}

\begin{Tool}{SimPARTIX}{partix}
TODO.
\end{Tool}

\begin{Tool}{SimulationX}{simulationx}
TODO.
\end{Tool}

\begin{Tool}{SIMULIA Co-Simulation Engine}{simulia}
TODO.
\end{Tool}

\begin{Tool}{SystemC}{systemc}
TODO.
According to \cite{Krammer2015a}, SystemC is a discrete event simulation.
It is used for modeling and simulation of digital software and hardware systems.
\end{Tool}

\begin{Tool}{SystemC/AMS}{systemc_ams}
According to \cite{Krammer2015a}, SystemC/AMS supports timed dataflow, linear signal flow and electrical linear networks.
\end{Tool}

\begin{Tool}{VDM}{vdm}
TODO.
\end{Tool}

\begin{Tool}{TEODACS FlexRayExpert.Sim}{teodacs_flexrayexpert_sim}
TODO.
\end{Tool}

\begin{Tool}{TINE}{tine}
TODO.
\end{Tool}

\begin{Tool}{TISC Suite}{tisc}
TODO.
\url{www.tlk-thermo.com}
According to \cite{Broman2013} they use a variable synchronization step size.
A simulation module can propose the length of the next time step.
\end{Tool}

\begin{Tool}{TLK FMI Suite}{tlk}
TODO.
\end{Tool}

\begin{Tool}{TWT Co-simulation Framework}{twt}
TODO.
\end{Tool}

\begin{Tool}{VLAB Co-simulation}{vlab}
TODO.
\end{Tool}

\begin{Tool}{VSM}{vsm}
TODO.
\end{Tool}

\begin{Tool}{WAVE}{wave}
TODO.
\end{Tool}

\begin{Tool}{xMOD}{xmod}
TODO.
\end{Tool}

\begin{Tool}{Aldec}{aldec}
TODO.
\end{Tool}

\begin{Tool}{CODIS}{codis}
TODO.
\end{Tool}

\begin{Tool}{Functional Digital Mock-up Framework}{FDMU_framework}
TODO
\end{Tool}
\begin{Tool}{Ptolemy II}{Ptolemy_II}
TODO
\end{Tool}
\begin{Tool}{Building Controls Virtual Test Bed (BCVTB)}{BCVTB}
TODO
\end{Tool}



==> state_of_art_unrelated.tex <==
\section{State of the Art in Co-simulation Not Classified}

Unrelated references are references that were covered, but are were not classified due to being either too broad or unrelated to co-simulation.


\begin{Reference}{Co-simulation of multibody and hydraulic systems: comparison of different coupling approaches}{Schmoll2011}
No access.
\end{Reference}


\begin{Reference}{Co-simulation Study of Vehicle ESP System Based on ADAMS and MATLAB}{Li2011a}
This work describes an application of co-simulation to the automotive domain.
\end{Reference}


\begin{Reference}{Towards a DSM-based framework for the development of complex simulation systems}{Li2011b}
This is about co-modelling.
\end{Reference}


\begin{Reference}{Generation of sparse jacobians for the function mock-up interface 2.0}{Akesson2012}
This work does not describe a co-simulation approach.
\end{Reference}


\begin{Reference}{An efficient unified method for the combined simulation of multibody and hydraulic dynamics: comparison with simplified and co-integration approaches}{Naya2011}
This is not about co-simulation.
\end{Reference}


\begin{Reference}{A Domain-Specific Language For Simulation Composition.}{Schutte2011}
This work describes a single simulator.
\end{Reference}


\begin{Reference}{A co-simulation framework for full vehicle analysis}{Datar2011}
No access.
\end{Reference}

\begin{Reference}{Implementation of Modelisar Functional Mock-up Interfaces in SimulationX}{Noll2011}
Discusses an implementation of FMUs.
\end{Reference}

\begin{Reference}{Using of Co-simulation ADAMS-SIMULINK for development of mechatronic systems}{Brezina2011}
This work describes an application of co-simulation.
\end{Reference}

\begin{Reference}{On the efficient coupling of simulation codes}{Busch2012a}
This is a PhD Thesis. The respective papers were classified.
\end{Reference}


\begin{Reference}{Functional mock-up interface in mechatronic gearshift simulation for commercial vehicles}{Abel2012}
This work describes an application of co-simulation to the simulation of gearshift in cars.
\end{Reference}


\begin{Reference}{Hybrid CPU-GPU Distributed Framework for Large Scale Mobile Networks Simulation}{Bilel2012}
This work introduces a new CPU-GPU co-simulation framework where synchronization and experiment design are performed on CPU and node's processes are executed in parallel on GPU according to the master/worker model.
This is not related to co-simulation as defined in this work.
\end{Reference}


\begin{Reference}{Collaborative Modelling and Co-simulation with DESTECS: A Pilot Study}{Pierce2012}
This work describes an application of the tool DESTECS for the development of a line following robot.

\end{Reference}


\begin{Reference}{Intelligent Design" Real-Time Simulation for Smart Grid Control and Communications Design}{Anderson2012}
This is a magazine article.
\end{Reference}

\begin{Reference}{A framework for simulation-based real-time whole building performance assessment}{Pang2012}
This work describes an application of co-simulation.
\end{Reference}


\begin{Reference}{An approach for the coupled simulation of machining processes using multibody system and smoothed particle hydrodynamics algorithms}{Spreng2013}

This work describes a co-simulation approach between two tools: Pasimodo and Simpack.
The coupling, called Neweul-M2, is done through output to input assignments but adaptations are necessary.

\catref{nfr:distribution}
\catref{sr:rollback:none}
\catref{sr:rel_time:analytic}
\catref{sr:causality:causal}
\catref{sr:info:full_model}
\catref{sr:availability:remote}
\catref{fr:alg_loop:explicit}
\catref{fr:domain:ct}
\catref{fr:coupling_model:io_assignments}
\catref{fr:num_sim:two}
\catref{fr:sim_rate:single}
\catref{fr:sim_step_size:fixed}
\catref{fr:results_visualization:post_mortem}

\end{Reference}


\begin{Reference}{Error Analysis and Error Estimates for Co-Simulation in FMI for Model Exchange and Co-Simulation V2.0}{Arnold2013}
This work studies the numerical error made in CT co-simulation.
\end{Reference}


\begin{Reference}{The FMI++ library: A high-level utility package for FMI for model exchange}{Widl2013}
This work describes an abstraction over the basic FMU, as described by the FMI standard.
An interesting feature is that it enhances the FMU's with the ability to provide predictable step sizes.
Unfortunately, this work is not related to FMI co-simulation and does not describe a master to be classified.
\end{Reference}



\begin{Reference}{A Comprehensive Approach for Modeling, Simulation and Virtual Validation of Integrated Safety Systems}{Karner2013}
This work shows how co-simulation enables a process for modeling, simulation and virtual validation of integrated safety systems. 
For that, it makes used of the ICOS tool.
ICOS is a co-simulation framework that currently supports more than 30 industrial simulation tools.

\end{Reference}

\begin{Reference}{A co-simulation method as an enabler for jointly analysis and design of MAS-based electrical power protection and communication}{Li2013}
This works presents a co-simulation platform that incorporates two tools: Virtual Test Bed and OPNET.
The tools is already described in \cite{Li2011c}.
The majority of the work is focused on a case study.
\end{Reference}


\begin{Reference}{Modelica-enabled rapid prototyping of cyber-physical energy systems via the functional mockup interface}{Elsheikh2013}
This work is an overview on the benefits and challenges of incorporating Modelica-based FMUs into other simulation languages.
\end{Reference}


\begin{Reference}{Co-simulation Solutions using AA4MM-FMI applied to Smart Space Heating Models}{Gilpin2014}

This work describes a co-simulation master for FMI, tailored for HVAC systems.
No enough details are provided about the co-simulation master to be classified.

\end{Reference}

\begin{Reference}{Co-simulation platforms for co-design of networked control systems: An overview}{Li2014}
This work reviews some co-simulation frameworks for the development of networked systems.
\end{Reference}


\begin{Reference}{Mixed-mode simulation and analog multilevel simulation}{Saleh2013}
This is a book about mixed-mode simulation.
In the introduction they give a bit of background on what they consider to be mixed mode simulation and the multiple levels of detail involved in the development of both analog and digital circuits.
From this explanation, it seems like mixed mode simulation does not fit in the definition of co-simulation but in other references it fits.
They discuss the advantages and the challenges of mixed-mode simulation.
They also introduce very informally 4 synchronization schemes: lock-step, digitally controlled, analog controlled and rollback based.
Since this definition is very high level, we are not able yet to discern these from the existing ones that we have already described.
They present three strategies to develop mixed mode simulators:
\begin{description}
\item[Core modification approach] - Extend existing simulators to become mixed mode simulators.
\item[Glue approach] - this is basically co-simulation. They present the simulation backplane technology as an enabler for this. The simulation backplane is basically a set of well defined interfaces for the communication between simulators (very similar to the FMI).
\item[Fully integrated approach] The definition suggests that the resulting simulation tool is much more integrated.
Comparing to the other two categories, this seems to be just a tool developed from scratch.
\end{description}
\claudio{This simulation backplane technology is the analogous to FMI in the mixed mode simulation realm.}
They conclude the introduction with a list of tools that performed mixed-mode simulation and their capabilities.
Chapter 2:
They give the basic theory behind numerical integration and fixed point techniques.
They start with the description of nodal analysis and an overview on the circuit simulation algorithm.
Then they discuss ways to control the time-step (theoretical and implementation) of the simulation according to three constraints:
accuracy, stability, and stiffness.
In terms of implementation, they describe two possible ways to control the time-step: directly according to the LTE, or according to the number of iterations of the fixed point technique.
\end{Reference}


\begin{Reference}{Design of modern vehicle electrical systems based on co-simulation and a model library}{Zehetner2013}
This describes an application of co-simulation.
Not enough details are provided about the co-simulation orchestration.
\end{Reference}

\begin{Reference}{Nonlinear State Estimation with an Extended FMI 2.0 Co-Simulation Interface}{Brembeck2014}
They describe a non-linear state estimation technique and not a co-simulation framework.
\end{Reference}

\begin{Reference}{Exact Method for Coupled Non-linear State-space Simulation and its Application to a Flexible Multibody Wind Turbine Aeroelastic Code}{Betran2014}
This work is based on how to decouple models, and not co-simulation.
\end{Reference}

\begin{Reference}{Control of an engine test-bench via hardware-software-co-simulation}{Zehetner2014}
We do not have access to this paper.
\end{Reference}

\begin{Reference}{Context-based polynomial extrapolation and slackened synchronization for fast multi-core simulation using FMI}{Khaled2014}
The work describes a techniques for the implementation of a simulator, using FMI for model exchange.
The essential idea of this work is to come up with a look up table of input extrapolator that can be used depending on the context. The context is given by comparing, say, the last three points. For example, they have two thresholds for the variation between the last three points. With those thresholds, they can distinguish between a signal that is a bump, from a signal that is mostly flat, or mostly linear. However, they have a very nice intuitive explanation of how the errors get propagated in the solution. Ah, they borrow a neat idea from image compression algorithms to build a lookup table that chooses the right extrapolation at any time, based on the pattern of signals. They present nice related work for signal extrapolation. They perform a derivation of least square error which I have to pay a closer attention to. Paper [17] is related work to our own. 
The big advantage of their work is that it is capable of working well with discontinuities. However, the way they compare their work with polynomial extrapolation is not entirely fair, and there is no reset of the state of the polynomial... They point to [21] as a good hint of future work.
\end{Reference}

\begin{Reference}{Co-simulation Environment for Rodin: Landing Gear Case Study}{Savicks2014}
It is a work in progress and does not provide enough detail.
\end{Reference}

\begin{Reference}{Simulating Rhapsody SysML Blocks in Hybrid Models with FMI}{Feldman2014}
This work describes the implementation of a single FMU to support the simulation of statchart.
The main challenges are highlighted.
\end{Reference}

\begin{Reference}{Tool coupling for the design and operation of building energy and control systems based on the Functional Mock-up Interface standard}{Nouidui2014}
This work gives recommendations on what tools to use to perform co-simulation of HVAC systems.
\end{Reference}

\begin{Reference}{Functional mock-up unit for co-simulation import in EnergyPlus}{Nouidui2014a}
This work describes the implementation of an FMU for FMI co-simulation and its subsequent application to HVAC.
\end{Reference}


\begin{Reference}{Consistent Simulation Environment with FMI based Tool Chain}{Drenth2014}
Describes an application of co-simulation without sufficient detail to be classified.
\end{Reference}

\begin{Reference}{Virtual Integration for hybrid powertrain development; using FMI and Modelica models}{Belmon2014}
This describes the application of co-simulation to powertrain development. 
It does not provide sufficient detail to be classified.
\end{Reference}


\begin{Reference}{Adapting Functional Mockup Units for HLA-compliant Distributed Simulation}{Ylmaz2014}
This work aims at wrapping an FMU into an HLA.
\end{Reference}

\begin{Reference}{Bridging the Semantic Gap Between Heterogeneous Modeling Formalisms and FMI}{Tripakis2015}
\cite{Tripakis2015} discuss how to create different FMUs from heterogeneous modeling formalisms. 
It formally defines how to encode an FMU and which adaptations are required for certain classes of formalisms, for example timed and un-timed formalisms (e.g., Statecharts).
There is an abuse of the standard however: the FMI standard does not allow for zero time computations.
\end{Reference}

\begin{Reference}{Co-Simulation of IP Network Models in the Cyber-Physical Systems Context, using a DEVS-based Platform}{Vaubourg2016}
This work proposes to integrate multiple IP simulators for the purpose of being used in cyber physical system simulation.
The co-simulation orchestration is the one in \cite{Camus2016} so this paper is not the co-simulation framework per se.
\end{Reference}

\begin{Reference}{On the integration of HLA and FMI for supporting interoperability and reusability in distributed simulation}{Garro2015}
This work describes the technical details behind an integration of FMI into HLA.
\end{Reference}

\begin{Reference}{Multi-domain Modelling in DESTECS and Ptolemy - a Tool Comparison}{Wolff2015}
This is a tool comparison paper.
\end{Reference}

\begin{Reference}{Iterative Simulation-Optimization of a Multi-State Manufacturing System}{Dehghanimohammadabadi2015}
Simulation optimization is an emerging field which is widely applied in various industries including manufacturing.
This is not related to co-simulation, although co-simulation can be used in it.
\end{Reference}


\begin{Reference}{Functional Development of Modern Control Units through Co-Simulation and Model Libraries}{Benedikt2015}
No details are provided about the co-simulation orchestration.
\end{Reference}

\begin{Reference}{A simulation of a power surge monitoring and suppression system using LabVIEW and multisim co-simulation tool}{Abad2015}
It describes an application of co-simulation to monitor power surges in distribution systems.
No details are provided about the co-simulation orchestration.
\end{Reference}

\begin{Reference}{Using FMI components in discrete event systems}{Muller2015}
The paper is based on \cite{Muller2013} and shows that the use of FMI components has better scalability and shorter runtime than a pure Ptolemy II implementation.
The comparison is based on an example consisting of a set of houses with heating. The temperature inside a house is given by a system of differential equations. The temperature inside the houses is controlled by an on-off controller, which switches between a min and max temperature.
Three runtimes are presented: One using pure Ptolemy II, one using Java FMU actors, and one using C++ FMU actors. A figure  shows a graph with the
execution time for different numbers of houses.
It is not considered in our classification because it provides a solver for the model, using FMU model exchange standard.

\end{Reference}


\begin{Reference}{A Co-simulation Platform of Integrated Starter/Generator System Based on ANSYS}{Zhang2016}
This work shows how the development of a integrated starter/generator system can be developed with the help of co-simulation.
No details are provided about the co-simulation orchestration.
\end{Reference}

\begin{Reference}{Co-simulation of Power System and Synchrophasor Communication Network on a Single Simulation Platform}{Gurusinghe2016}
It describes a case study in power systems.
It does not provide enough detail to understand and classify the co-simulation framework.
\end{Reference}

\begin{Reference}{Collaborative Model-based Systems Engineering for Cyber-Physical Systems -- a Case Study in Building Automation}{Fitzgerald2016}
It describes a case study in HVAC.
It does not provide enough detail to understand and classify the co-simulation framework.
\end{Reference}

\begin{Reference}{A Model-driven and Tool-integration Framework for Whole Vehicle Co-simulation Environments}{Lu2016}
They describe a co-simulation framework that couples Carmaker, MWorks and Simulink.
There are several flaws in the paper which make it hard to read. This includes unreadable pictures.
\end{Reference}

\begin{Reference}{The high level architecture RTI as a master to the functional mock-up interface components}{Awais2013}
The article describes an experiment, where a High Level Architecture (HLA) compliant Run Time Infrastructure (RTA) is used for running simulations
with FMUs. The experiment consists of two balls than can collide. It is described how to pass data, the federate object model, and
an algorithm for doing time advances. Furthermore, it contains ideas on how to use Interoperability Reference Models (IRM) for the FMI standard. IRMs
provide a structured way of comparing capabilities of any interoperability or co-simulation standard. However, the FMI is quite different from other
interoperability standards, as these work with processes whereas FMI works with libraries. The only describe it in a time-stepped fashion without
events, as FMI cannot provide precise timestamps for events.

This does not describe a framework but a possible approach on how to integrate FMI when using HLA.
\end{Reference}


\begin{Reference}{Hardware/software cosimulation from interface perspective}{Yoo2005}
	The paper presents an overview of abstraction levels used in mixed-level cosimulation and is in general a good overview of HW/SW cosimulation. Furthermore it introduces the term ``Refinement space'' and uses it along with the concept ``HW/SW interface'' to describe mixed-level cosimulations.
	The article does not present new ideas except refinement space, but explains current issues in HW/SW cosimulation. This also includes cases where HW modules with different abstraction levels communicate with each other. It also addresses raising abstraction levels to improve performance.
\end{Reference}

\begin{Reference}{Standard compliant co-simulation models for verification of automotive embedded systems}{Krammer2015a}
They describe the implementation of FMI support for the tools SystemC and SystemC/AMS.
The support is done by coding a wrapper component that adapts the executable code generated by the tools and turns it into an FMU.
They test their wrappers by performing a co-simulation using the \toolref{icos} tool, which gives us more details about the tool.
\end{Reference}


\begin{Reference}{Significant Reduction of Validation Efforts for Dynamic Light Functions with FMI for Multi-Domain Integration and Test Platforms}{Schneider2014}
Based on FMI.
Touches upon X-in-the-loop co-simulation.
They give an overview of the CarMaker tool but not enough detail to be classified.
\end{Reference}

\begin{Reference}{On the difficulties of real-time co-simulation}{Stettinger2013a}
They address real-time co-simulation.

They identify the three main challenges in CT co-simulation:
Pick the right coupling time instants;
Select the appropriate extrapolation method; and
Define the sub-system scheduling policy.
In general, there is the accuracy/performance tradeoff with the co-simulation step size.
They identify the following challenges in real-time co-simulation:
- All simulators have to be fast enough to fullfil the real-time deadlines. In this case, the synchronization is made by slowing down the simulators.
- Dead time elimination. This is related to the delays in the communication of samples. To ensure that the real-time systems gets inputs in a timely order, an extra coupling component is added to compensate for any delayed sample.
- Extrapolation of noisy signals. In this context, the old extrapolation functions cannot be used, and other techniques that deal with noisy signals, such as Kalman filtering, have to be used.
They also show that, once you go into hierarchical co-simulation, scheduling becomes an interesting problem, because you may want to combine jacobian scheduling at the top level, nad gauss seidel at the lower levels. Have a measure of the worst case execution time for each simulator plays a fundamental role in evaluating the different approaches.

Overall the paper is a summary of what has been done in the journal publication: \cite{Stettinger2013}.
\end{Reference}

\begin{Reference}{Generation of Functional Mock-up Units for Co-simulation from Simulink Using Explicit Computational Semantics: Work in Progress Paper}{Pussig2014}
This work is about the generation of FMU's from Causal Block Diagram models.
\end{Reference}

\begin{Reference}{A Comparative Study of Mixed Mode Simulation Methods : Approaches in Research and Practice}{Gandhi2015}
This is a survey of simulation tools used in HVAC. What is interesting is that most of the surveyed works want to have better integrated simulation tools. This is because introducing the same data in both tools takes time and may cause errors. Another of the asked features was the capability to visualize information. This is again related to co-simulation: an individual simulator knows best how to plot the data from its own domain. They also ask for tools that better support an iterative development.
However, there is little information about the tools used in this reference.
\end{Reference}

\begin{Reference}{Can complex systems really be simulated?}{Kalmar-Nagy2014}
They study the stability with multiple coupling approaches in co-simulation (gauss seidel, jacobi and iterative jaccobi). They make the following assumptions: 
- Force/displacement approach
- The sub-systems each use a RK4 method and ONLY one time step is performed.

They conclude that under these assumptions, not surprisingly, gauss seidel and strong coupling (iterative jacobi) are the best methods in terms of stability properties. 

In general the paper is a good read in terms of learning the basics of continuous time co-simulation.
\end{Reference}

\begin{Reference}{Explicit and Implicit Cosimulation Methods: Stability and Convergence Analysis for Different Solver Coupling Approaches}{Schweizer2015c}

It is hard to tell the difference between this paper, and the others from the same author.
It appears that no new methods are proposed in this paper. Only existing ones are studies.

\end{Reference}

\begin{Reference}{Toward an Hybrid Co-simulation with the FMI-CS Standard}{Tavella2016}

This is a report.
It is related to DACCOSIM.
They describe further extensions to the FMI standard in order to support hybrid system simulation. They suggest a new function for easing the tracking of events in the FMI.

Seems very preliminary work to be classified.
\end{Reference}

\begin{Reference}{From AUTOSAR Models to Co-simulation for MiL-Testing in the Automotive Domain}{Mews2012}
Based on SIMULINK and therefore not a co-simulation framework or master per se.
According to \cite{Krammer2015}, a test setup modeling language (TSML), analogous to a co-simulation description language, which aims at model-in-the-loop simulation.

The paper describes a test setup modeling language that can describe test-setups for co-simulation. The TSML (Test Setup Modeling Language) can model the relevant pieces in a tool-independent manner. 

The architecture of TSML is described along with a thorough description of the steps involved
in creating a TSML instance for MiL testing based on AUTOSAR. Furthermore it is described how to achieve the tool-independent behavior, which is
carried out by using adapters for the various tools.

The article also describes the entire workflow by an example application based on automotive direction indicator system.

Furthermore, the article also introduces MiL, AUTOSAR, and MiL-testing. 

Since it was part of the MODELISAR project it is finished in 2011?! \url{https://itea3.org/project/modelisar.html}
The project is also part of virtuOS, however data on this project is difficult to find. It seems like it was also part of MODELISAR.
Because the project seems to be finished without any additional articles and similar I do not think it is worth using any more resources on.
However, it is worth referencing.

\end{Reference}



\begin{Reference}{Challenges in Automotive Software Engineering}{Broy2006}
Gives an overview of software development in the automotive industry.
As one might expect, they focus exclusively on the software development and little on the hardware development.
So it is not of much use.

Arguments in favor of co-simulation.
It is one of the enablers of seamless model driven development at all levels. Not just software but also hardware.
They talk about a limit on the combinatorial complexity of languages and tools for the development of cars.
Co-simulation can also contribute to the support of this heterogeneity.
\end{Reference}


\begin{Reference}{Zero-crossing location and detection algorithms for hybrid system simulation}{Zhang2008}
They discuss the challenges involved in the location and detection of zero-crossing.
They also make clear the need for compositionality in co-simulation, that is threatened by the zero-location algorithms.
They start with the challenges in detecting a zero crossing: even-roots, double detection and masked even roots (the compositionality problem).
Once detected, the precise time of the events need to be located.
They focus on zero-crossing location when Zeno behaviors occur.
To show the effectiveness of the approach they propose to solve the problem with Zeno behavior, they use a double bouncing ball in stairs as an example.
This is neither a co-simulation framework nor a synchronization scheme.
\end{Reference}

\begin{Reference}{Semi-formal Modeling of Simulation-based V \& V Methods to Enhance Safety}{Krammer2014}
In \cite{Krammer2014}, Krammer et al. propose a language (ICOSdl) to describe co-simulation scenarios. 
The language is based on a set of UML profiles.
This language reduces the effort in the configuration of complex scenarios.
An air-bag system co-simulation scenario is used to validate the language.
It couples Simulink models with a CarMaker model.
It is not clear where are the simulators being coupled in their approach.
They only talk about co-simulation scenarios.
They motivate the need for reusing the configuration parameters of co-simulation units (e.g., a co-simulation model might be instantiated in a co-simulation scenario multiple times). 
The solution for this can be class-based inheritance for co-simulation units or prototype based (as in Javascript).
After the simulation scenario is described, the ICOS tool (\toolref{icos}) is used to execute the co-simulation.
\end{Reference}

\begin{Reference}{Efficient Master/Worker Parallel Discrete Event Simulation on Metacomputing Systems}{Park2012}
This concerns parallel discrete event simulation.
\end{Reference}

\begin{Reference}{Efficient Master/Worker Parallel Discrete Event Simulation}{Park2009}
This concerns parallel discrete event simulation.
\end{Reference}

\begin{Reference}{Analog and mixed signal modelling with SystemC-AMS}{Vachoux2003}
This paper introduces concepts for the extension of the SystemC methodology for the specification and design of analog and mixed signal systems.
\end{Reference}

\begin{Reference}{Capturing the dual relationship between simulation models and their context}{Traore2006}
Seems to give a nice introduction to modeling and simulation (and experimental frames).
\end{Reference}

\begin{Reference}{Symbolic analysis of electronic circuits based on a tree enumeration technique}{Sharif-Bakhtiar1993}
Seems they infer transfer functions by analyzing the circuits.
I'm not sure we can use something from this.
\end{Reference}

\begin{Reference}{VHDL-AMS and Verilog-AMS as alternative hardware description languages for efficient modeling of multidiscipline systems}{Potop-Butucaru2005}
The paper compares two languages.
\end{Reference}

\begin{Reference}{Distributed Discrete-event Simulation}{Misra1986}
Presents a survey on distributed event simulation algorithms.
\end{Reference}

\begin{Reference}{Global Optimization of Algorithms}{Mitsos2008}
This citation points to a lecture.
\end{Reference}

\begin{Reference}{Standards for system-level design: practical reality or solution in search of a question?}{Lennard2000}
They present an three standards in the system-level VC integration space, and describe two distinct industrial case studies to support their practicality.
\end{Reference}

\begin{Reference}{The Waveform Relaxation Method for Time-Domain Analysis of Large Scale Integrated Circuits}{Lelarasmee1982}
They present the Waveform Relaxation method: an iterative method for simulating nonlinear dynamical systems in the time domain.
According to \cite{McCalla1987}, the waveform relaxation is based on generalizing the Gauss-Seidel and Gauss-Jacobi relaxation techniques to solve a complete signal instead of just one value.
This gives us ideas about the categorization but it is not directly related to co-simulation.
\end{Reference}

\begin{Reference}{Simulation Modeling and Analysis}{Law2000}
A book mostly focused on Simulation from the Operations Research point of view.
\end{Reference}

\begin{Reference}{Modeling and simulating optical MEMS using Chatoyant}{Kurzweg1999}
They present Chatoyant, which is a mixed-signal opto-electronic simulation framework built on top of ptolemy.
Does not seem to be related to co-simulation.
\end{Reference}

\begin{Reference}{A Hardware-Software Codesign Methodology for DSP Applications}{Kalavade1993}
They describe a systematic, heterogeneous design methodology using the Ptolemy framework for simulation, prototyping, and software synthesis of systems containing a mixture of hardware and software components.
\end{Reference}

\begin{Reference}{VHDL-AMS - A hardware description language for analog and mixed-signal applications}{Christen1999}
Provides an overview of the VHDL-AMS hardware description language.
\end{Reference}

\begin{Reference}{Multidisciplinary modelling and simulation speeds development of automotive systems and software}{Chombart2012}
\cite{Chombart2012} reports on the impact that the MODELISAR project has had in
the industry.
Some 34 FMI-compatible tools have been announced with 25 of them available
commercially.
Industrial partners are starting to exploit FMI as a fast and efficient way to
exchange virtual prototypes between teams.
Daimler intends to use FMI in future gearbox projects for Mercedes-Benz cars.
And FMI should become the standard interface for model exchange and simulation
tool coupling in software-in-the-loop simulations at Daimler Trucks Customer
Application Engineering, especially for power-train dynamics.
Dassault Systèmes is integrating MODELISAR developments in the CESAR project:
the Enovia Reference Technology Platform for CESAR leverages MODELISAR results,
particularly the capability to handle AUTOSAR models, C Code and FMU description
files.
The consolidated results of CESAR and MODELISAR will offer a larger scope for
systems engineering activities.
TWT is focusing on shared simulation incorporating FMI in the iSSE CleanSky
project.
By co-simulating static and dynamic performance of on-board aircraft systems,
the concept of an all-electric aircraft can be comprehensively assessed with
particular focus on electrical power absorption and thermal energy production.
\end{Reference}

\begin{Reference}{Heterogeneous Simulation—Mixing Discrete-Event Models with Dataflow}{Chang1997}
This is about semantic adaptation between discrete event models and dataflow.
\end{Reference}

\begin{Reference}{Context-sensitive synthesis of executable functional models of cyber-physical systems}{Canedo2013}
Functional Modeling (FM) is a Systems Engineering methodology where products are
initially described in terms of their functionality \cite{Canedo2013}.
Because the descriptions contain only what the products do - as opposed to how
they do it - FM improves the communication between different engineering teams
allowing for a more integrated development of mechatronic systems.
The approach followed in \cite{Canedo2013} attempts to support FM and enable
integrated development of complex systems by automatically generating
multi-domain, simulation-ready, Modelica models from Functional Basis models.
However, as is shown in \cite{Zeigler2000}, there is not enough
information to, in the general case, infer the correct structure of the system
from its functional specification. Even is that was possible, one still must
also account for non-functional requirements (performance, cost, robustness,
etc\ldots). That is why they develop an algorithm that attempts to infer the
context in which a functional specification is and, together with good
engineering heuristics, generate simulation models that reuse already developed
components.
The context is inferred from the connections going in and out of each functional
model. Their code generator also accommodates human provided inputs or, in their
terms, engineering views. Their approach is exemplified by generating the models
of a popcorn machine.
This is not related to co-simulation.
\end{Reference}

\begin{Reference}{Ptolemy II - heterogeneous concurrent modeling and design in Java}{Brooks2005a} 
Ptolemy will not be considered a co-simulation framework.
\end{Reference}

\begin{Reference}{The Functional Mockup Interface-seen from an industrial perspective}{Bertsch2014}
\cite{Bertsch2014} shows that some of the tools that claim to perform
co-simulation, actually have errors.
They evaluate some of those tools and they have identified five kinds of errors
according to their source:
\begin{enumerate}
  \item Inconsistencies in the standard;
  \item Formal errors in the FMU;
  \item Import of the FMU;
  \item Simulation of one FMU;
  \item Simulation of multiple FMUs;
\end{enumerate}
The last two kinds of errors are the ones we want to address in this PhD.
They motivate the need for a standardized way of describing co-simulation scenarios such that the errors that arise when simulating multiple FMU's can be checked.
\end{Reference}

\begin{Reference}{Formal verification of hybrid systems}{Alur2011}
They give a review of the approaches for formal verification of hybrid systems.
\end{Reference}

\begin{Reference}{A modular formal semantics for Ptolemy}{TRIPAKIS2013}
They propose the semantics of Ptolemy that are closed under composition.
This would fit in the Compositionality non-functional requirement but we are not considering Ptolemy to be a co-simulation framework.
\end{Reference}

\begin{Reference}{Leveraging synchronous language principles for heterogeneous modeling and design of embedded systems}{Lee2007a}
This is related to the composition of models of computation.
While it is relevant for co-simulation, I'm not sure it qualifies as a co-simulation framework.
\end{Reference}

\begin{Reference}{A Generic Execution Framework for Models of Computation}{Hardebolle2007}
They present a language for describing model of computation.
\end{Reference}

\begin{Reference}{Cyber-Physical Systems Design: Formal Foundations, Methods and Integrated Tool Chains}{Fitzgerald2015}
They seem to focus on the development of a tool chain for CPS.
\end{Reference}

\begin{Reference}{Semantic Adaptation Using CCSL Clock Constraints}{Boulanger2012}
This is related to semantic adaptation.
Even though semantic adaptation is closely related to accuracy of a co-simulation, we will consider this to be outside the scope of this review.
\end{Reference}

\begin{Reference}{Semantic Adaptation for Models of Computation}{Boulanger2011}
In \cite{Boulanger2011} they show how the power window example can be modeled
using computed languages.
They give examples for each kind of semantic adaptation:
\begin{description}
\item[Data] - different simulation units have different data structures and work with different signals.
\item[Time] - different simulation units have different notions of time (e.g., reals or integers).
\item[Control] - different simulation units may work at different rates with ones executing periodically and others executing sporadically.
\end{description}
The interface blocks are programed in Java, which is an error prone process.
\end{Reference}

\begin{Reference}{Simulation of Multi-Formalism Models with ModHel'X}{Boulanger2008}
Boulanger et al.~\cite{Boulanger2008} presents a framework, ModHel'X, for semantic adaptation of heterogeneous models by allowing the user to program an interface block between a main model and an embedded model.
This block adapts data, control and time so as to ensure that the embedded and the main model can be simulated correctly together.
The adaptation in ModHel'X is done at the model level, whereas in our work the focus is on the adaptation of the simulators.
This means that the composed language is created, and the modeler uses it without any concern about its semantics.
ModHel'X is not considered a co-simulation framework because there is no notion of independent simulators being coupled.
\end{Reference}

\begin{Reference}{Systems of Systems Engineering: Basic Concepts, Model-Based Techniques, and Research Directions}{Nielsen2015}
This provides a nice review of SoS research.
They start with a review on the definitions of SoS.
Based on those multiple definitions, they propose eight dimensions:
Autonomy, Independence, Distribution, Evolution, Dynamic Reconfiguration, Emergence of Behavior, Interdependence, and Interoperability.
They then table the definitions proposed by the literature to sets of these dimensions.
In section 4, they provide illustrative examples of SoS.
In section 5, they describe the state of the art in terms of modeling, simulation, testing and verification of SoS.
They conclude describing the main challenges in the research and development of SoS in the four aspects of the previous section.
\end{Reference}

\begin{Reference}{Large-scale network simulation: how big? how fast?}{Fujimoto2003}
They seem to focus on testing two network simulation tools and evaluating them in terms of number of packets processed per (wall clock) second.
\end{Reference}

\begin{Reference}{Operational semantics of hybrid systems}{Lee2005}
They describe the HyVisual tool which does not qualify as a co-simulation tool.
This tool uses the tagged signal to represent, for instance, the evolution of fixed point computations.
They also describe some of the challenges in handling discontinuous in traditional continuous time signals.
\end{Reference}

\begin{Reference}{The Functional Mockup Interface for Tool independent Exchange of Simulation Models}{Blochwitz2011}

This paper is not related because it is not a co-simulation framework.

Essentially they present the FMI Standard (version 1.0).
They introduce the two parts of the standard: model exchange and co-simulation.
In Section 2, they present the general ideas and motivation behind the FMI and some of the technical aspects of the distribution of the co-simulation units.
In Section 3 they describe the first part of the standard: the model exchange.
In Section 4, they turn to the co-simulation.
They describe the master/slave principle and examples of co-simulation scenarios that include the distributed ones, showing that the standard is quite flexible in terms of scenario complexity.
In Section 5 they compare multiple proprietary model-exchange formats with respect to multiple criteria.
In Section 6, they give a list of tools that support the FMI.
They conclude in Section 7 by reporting on the acceptance degree of the standard and present the next planned tasks.
\end{Reference}

\begin{Reference}{Functional Mockup Interface 2.0: The Standard for Tool independent Exchange of Simulation Models}{Blochwitz2012}
Essentially, they describe FMI 2.0.
Some of the differences between 2.0 and 1.0 are discussed: tunable parameters, causality information, Jacobian information and units description.

\end{Reference}

\begin{Reference}{Linking FMI-based components with discrete event systems}{Muller2013}
The paper describes how to use FMI for model exchange in Ptolemy II, which enables the import of models written by other tools.
An approach is presented that uses predictions for every continuous subsystem, and thereby these can be used as discrete components in a discrete event system.
This approach is implemented with FMUs (Model-Exchange) generated by OpenModelica and uses the Discrete Event domain of Ptolemy II as a proof of concept.
It's not co-simulation because the FMUs exported do not include their own solver.
\end{Reference}


\begin{Reference}{Holistic Simulation of FlexRay Networks by Using Run-time Model Switching}{Karner2010b}
This paper describes model switching in the TEODACS project and is therefore closely related to \cite{Karner2010} and \cite{Karner2010a}.
Besides introducing model switching the paper also describes some implementation details and when it is a good time to perform the model switching.
Furthermore, calculations are provided for calculating the achieved simulation performance from applying model switching. Finally an experiment is
conducted and the results are presented. One of these results caused an error, because the the network topology was changed.
\toolref{teodacs_flexrayexpert_sim}

As this tool is already presented and described in the reference for Heterogeneous co-simulation platform for the efficient analysis of FlexRay-based automotive distributed embedded systems it will not be described further here.
\end{Reference}

\begin{Reference}{FMI for Co-Simulation of Embedded Control Software}{Pedersen2016}
Application: Maritime environment
The paper presents a need for co-simulation with the objective of enhance the modelling development and distribution at MAN Diesel \& Turbo. This is founded in an increasing complexity of the traditional two-stroke diesel engine because of tougher legislation on pollution and a demand for support of alternative fuel types.

The framework Ptolemy II is used as co-simulation framework and FMUs are used as simulation units.
The main challenge is adapting the embedded engine control system into an FMU. Furthermore, the importance of configuration complexity/simplicity is stressed, as the system is to be used by different disciplines.

Having each discrete controller in its own FMU FMUs resulted in a slow simulation speed they were grouped into one fmu.
The article also describes how a common notion of time was achieved when simulation the network communication.
FMUs are used to wrap an x86 RTOS.
The example presented in the paper is the dynamics and control of heating up the SCR reator.
\end{Reference}

\begin{Reference}{A co-simulation environment for high-fidelity virtual prototyping of vehicle systems}{Datar2012}
Application: Automotive
The paper describes the current state of the art in vehicle virtual prototyping and the motivation for using it.
A limitation in the prototyping is a simulation environment that analyses the vehicle model together with the accurate powertrain models. The integration of vehicle body, tyre, powertrain, driver, and terrain into one simulation environment is the contribution of this paper. 
The integration of these key components makes it possible to gain insight into how the vehicle dynamics affect fuel consumption, chemical composition of emission, and vecihle control strategies.
The vehicle without powertrain is modelled with ADAMS and the PSAT is selected for powertrain simulations. To combine these it is necessary to create an interface between them. The connection between them is established in a SIMULINK environment by generating simulink models of both the ADAMS vehicle and the PSAT powertrain. FTIRE is used to capture the tyre-road interaction.

The framework is used in an experiment where different vehicle chassies masses are tested against a certain profile of acceleration/breaking.
The fuel economy for the different masses is also shown. 
Another experiment is also conducted with a US HMMWV on off-road terrain where the suspension stiffness effect on fuel economy is investigated

This described a way to combine the tools and thereby presents a methodology, but it does not propose a new co-simulation framework.
\end{Reference}

\begin{Reference}{Virtual Prototyping of Ground Vehicles}{Datar2007}
This technical report describes how to set up a co-simulation using the methodology also described in \cite{Datar2012}. 
\end{Reference}

